DEUP: Direct Epistemic Uncertainty Prediction

Epistemic Uncertainty is a measure of the lack of knowledge of a learner which diminishes with more evidence. While existing work focuses on using the variance of the Bayesian posterior due to parameter uncertainty as a measure of epistemic uncertainty, we argue that this does not capture the part of lack of knowledge induced by model misspecification. We discuss how the excess risk, which is the gap between the generalization error of a predictor and the Bayes predictor, is a sound measure of epistemic uncertainty which captures the effect of model misspecification. We thus propose a principled framework for directly estimating the excess risk by learning a secondary predictor for the generalization error and subtracting an estimate of aleatoric uncertainty, i.e., intrinsic unpredictability. We discuss the merits of this novel measure of epistemic uncertainty, and highlight how it differs from variance-based measures of epistemic uncertainty and addresses its major pitfall. Our framework, Direct Epistemic Uncertainty Prediction (DEUP) is particularly interesting in interactive learning environments, where the learner is allowed to acquire novel examples in each round. Through a wide set of experiments, we illustrate how existing methods in sequential model optimization can be improved with epistemic uncertainty estimates from DEUP, and how DEUP can be used to drive exploration in reinforcement learning. We also evaluate the quality of uncertainty estimates from DEUP for probabilistic image classification and predicting synergies of drug combinations.

==> figs/bias_variance_bis.tex <==
\begin{tikzpicture}
    \draw[smooth cycle, color=orange!30, fill=orange!30, very thick, tension=0.3] plot coordinates{(5,1) (4,-1) (-1,-2) (-5,0) (0,2)} node[black] at (-3,1.5) {$\mathcal{S}$};
    \draw[smooth cycle, color=gray!50, fill=gray!50, very thick, tension=0.3] plot coordinates{(3,0.6) (2.4,-0.6) (-0.6,-1.2) (-3,0) (0,1.2)};
    \fill[blue!20] (0.75, 3.25) ellipse (1.5 and 0.5);
    \draw[black, thick, dashed, -stealth] (-0.75, -0.25) -- (0.67, 0.2);
    \draw[black, thick, -stealth] (0.75, 0.25) -- (0.75, 3.15);
    \draw[black, thick, dashed] (1.6, 3.5) -- (0.75, 3.25);
    \draw[black, thick, dotted] (-0.75, -0.25) -- (0.75, 3.25);
    \filldraw[black] (-0.75, -0.25) circle (2pt) node[anchor=east] {$\hat{f}$};
    \filldraw[black] (0.75, 0.25) circle (2pt) node[anchor=west] {$\tilde{f}$};
    \filldraw[black] (0.75, 3.25) circle (2pt) node[anchor=east] {$f^*$};
    \filldraw[black] (1.6, 3.5) circle (2pt) node[anchor=west] {$y$};
    
    
    \node at (1.25,2.2) {bias};
    \node at (0.5,2.2) {$b$};
    \node at (0, 0.3) {$\Delta f$};
    \node at (0.5, -0.2) {$\approx$std. dev.};
    \node at (1, 3.6) {noise};
    \node at (-0.35, 1.5) {$\varepsilon(\hat{f})$};
\end{tikzpicture}


==> figs/bias_variance_figure.tex <==
\begin{tikzpicture}
    \draw[smooth cycle, color=orange!30, fill=orange!30, very thick, tension=0.3] plot coordinates{(5,1) (4,-1) (-1,-2) (-5,0) (0,2)} node[black] at (-3,1.5) {$\mathcal{S}$};
    \draw[smooth cycle, color=gray!50, fill=gray!50, very thick, tension=0.3] plot coordinates{(3,0.6) (2.4,-0.6) (-0.6,-1.2) (-3,0) (0,1.2)};
    \fill[blue!20] (0.75, 3.25) ellipse (1.5 and 0.5);
    \draw[black, thick, dashed, -stealth] (-0.75, -0.25) -- (0.67, 0.2);
    \draw[black, thick, -stealth] (0.75, 0.25) -- (0.75, 3.15);
    \draw[black, thick, dashed] (1.6, 3.5) -- (0.75, 3.25);
    \draw[black, thick, dotted] (-0.75, -0.25) -- (0.75, 3.25);
    \filldraw[black] (-0.75, -0.25) circle (2pt) node[anchor=east] {$\hat{f}$};
    \filldraw[black] (0.75, 0.25) circle (2pt) node[anchor=west] {$f$};
    \filldraw[black] (0.75, 3.25) circle (2pt) node[anchor=east] {$f^*$};
    \filldraw[black] (1.6, 3.5) circle (2pt) node[anchor=west] {$y$};
    
    
    \node at (1.25,1.75) {bias};
    \node at (0.5,1.75) {$b$};
    \node at (0, 0.3) {$\Delta f$};
    \node at (0.5, -0.2) {variance};
    \node at (1, 3.6) {noise};
    \node at (-0.35, 1.5) {$\varepsilon(\hat{f})$};
\end{tikzpicture}


==> rebuttal <==
Reviews: https://openreview.net/forum?id=eGLdVRvvfQ&noteId=CA6ItEZ4el

>>  Reviewer MM5Y (Second exchange):

Answer (for all reviewers - including this one ?): Thank you for your thorough feedback. Following your recommandations, we updated the manuscript, providing more details and additional references where needed, and clarifying other parts of the text. We removed the right part of Figure 2 and tried to explain H' differently in Section 2.3. We also added an ablation study in the appendix on the usefuleness of the stationarizing features in the SMO experiment, and updated Table 6 with more ablations. In the updated manuscript, the modifications with respect to the initially submitted version are in red. We would be happy to address any additional questions and concerns you might have.

Reviewr: The zero vector is generally not attainable by models that output softmax predictions. The SNGP paper shows that a uniform prediction is optimal for OOD. Further, how do you compute the NLL when your target vector is the zero vector? NLL == CrossEntropy and we take it over the target distribution (which usually is one-hot).

Could you clarify, please? Either way, this might need to be explicitly explained in the paper.

Also for OOD detection, it would not really matter how well OOD samples' "generalization error" and predicted uncertainty correlate. It would be more interesting to see how well predicted uncertainty predicts the generlization error for ID data because epistemic uncertainty should also tell us something about that.

Answer:
Thank you for raising this point. As we state in Section 5.3.2, we consider a per-class Binary Cross Entropy rather than a standard multi-class Cross Entropy. This is following prior work from van Amersfoort et al., (2020). So it is straightforward to compute the NLL even with a zero target vector. Note that this NLL is computed only for evaluation, but in practice, we simply use the uncertainty predicted by DEUP to make the decision. We clarified this in the updated manuscript, and rewrote that section by incorporating more details that were in the appendix. 

We believe the correlation between the generalization error and predicted uncertainty is useful for 2 reasons:
a) It allows us to measure how reliable the uncertainty estimates generalize out-of-distribution. This is critical in interactive decision making where we want the uncertainty estimates to be accurate on out-of-distribution points to acquire the most informative ones. 
b) The "difficulty" of all OOD examples is not the same. For example, for a model trained on images of particular species of cats and dogs, an image of a different species is less "difficult" than an image of a car. 

Reviewer: Thanks for this. Let's discuss this a bit to improve the text potentially.

    You define the hypothesis space as the subset from the functions from without taking into account the data. That is, you define it as the possible hypothesis space prior to knowing about any data. It is the prior hypothesis space. You then use empirical risk minimization to find
    
    The prior hypothesis space is data-independent by definition. There is no that changes as

Hence, your arguments are not clear. You talk about the "reachable" hypothesis space in the text and refer to Figure 2, but that is not what the prior hypothesis space is as defined in the paper.

It would seem that you at some point switch from the prior hypothesis space to a "sort-of" prior-posterior hypothesis space that is reachable through SGD and randomness (even though there might only be a few global solutions in general) given data, but that is not prior to receiving data, but it is not clear.

More generally, is any of this really needed in the paper? Given your definition of the hypothesis space, my confusion would seem understandable, and there is no as depicted in Figure 2.

Please update Figure 2 and clarify and simplify the text as feasible.

Answer:
Thank you for engaging in this interesting discussion. 
Let's take the example of Deep Learning: The hypothesis space H is defined not only through the chosen architecture of the network, but also through the pre-defined training procedure (e.g. the hyperparameters of
the optimizer, the stopping criterion based on the performance on a validation set chosen from the training
data...). This means that even though the learning strategy is data-independent, the (reachable) hypothesis space H
depends on the training data. Arpit et al. (2017) formalized this subtle distinction using the notion of
“effective capacity”. As a consequence, the learner can incorporate new training examples in areas of the input
space where the bias is large, in order to change the hypothesis space H to H′, which can be closer to the
Bayes predictor, thus reducing the bias, and de facto the excess risk ER.

We believe that a key contribution of our work is that it takes into account that the family of function can grow in size (and thus bias be reduced) as more data becomes available, in order to estimate a reducible uncertainty that includes the effect of such bias reductions. 

Following your recommandation, in the udpated manuscript, we removed the right part of Figure 2, and added this explanation about how more data can shift the hypothesis space in Section 2.3.


Reviewer: As mentioned in my requested changes, an ablation is needed for this. Especially to motivate the claims and how this is different from the prior art (the collection of statistics papers). Novelty is not a requirement for acceptance, but the validity of claims is.

At the very least, it would be good to see an ablation for the different subsets of the four features, e.g. an extended Table 6 from the appendix.

In particular, if you only used
as the feature for training , the expectation would be that reports high loss everywhere, given the nature of how you probably select new samples. BTW could you add an example of
\pi(. \mid h_D, ...) to the main paper?
to the main paper?

I still don't understand why x by itself is a good idea.

If this is commonly done in pre-deep learning literature, could you add such references and citations to the paper for me to check?

Thanks!

Answer: 
We added two sentences before Algorithm 3 providing examples of acquisition functions $\pi$. 
We also added a few sentences after Equation 12 explaining that using x alone is not a good idea, and refering to the ablation in Table 6, in addition to the new ablation study we peformed with different subsets of the features in one of the SMO experiments. This new ablation shows that having x *in addition to* some of the other features might be helpful. We also added ablations with x as a feature in Table 6.


Reviewer: I am not sure if that is the right direction because what you describe is active learning, and in a changed revision you would have to make clear how "interactive learning" is different from "active learning" and why you don't compare to it. Also given that some prior art does use such approaches in active learning settings.

Given the other point ((11)->(12)), this may be a lower priority, but if you want to make this paper as impactful as possible, I would highly suggest running an active learning experiment on some datasets... MNIST and CIFAR-10 or CINIC-10 maybe?

Answer: 


In the updated manuscript, we removed all references to active learning, and only refer to "interactive learning". We use interactive learning as a general setting of which classical active learning, SMO and RL are particular instantiations of. We believe two of our sets of experiments (SMO, RL) should serve as enough evidence for the claims we make. 






----------------------------------------
>> Reviewer iZLw


Thank you for your detailed feedback.

* We would like to first address your concern about the “fit-the-fit” approach:
    - Similar to the referenced work "Density of States Estimation for Out-of-Distribution Detection” (that we were not aware of — we will add it the Related Work section), DEUP does not assume access to OOD data. While Figure 1 might give the impression that a validation set is necessary, this is merely a pedagogical example to introduce DEUP. Our focus is on interactive settings, where OOD data is “free”: the data obtained at a certain timestep before the main predictor is trained on it. We will emphasize in the introduction that no OOD data, nor withheld training data / validation data, is necessary in the settings of interest.
    - Unlike the referenced work, OOD detection is merely an instance of the myriad of tasks that would benefit from accurate uncertainty estimation. In particular, we evaluate DEUP on active learning settings, where high epistemic uncertainty should drive more exploration.
    - The comment "If on in-data one finds the fit to be poor, then this suggests the underlying model could be improved. If one knows the definition of OOD then one could train a classifier directly to train it.” does not necessarily apply to interactive settings. The fit can be perfect on a given dataset, but then the learner can be “surprised” by a poor fit on new examples. As is common in active learning and SMO, such a scenario should encourage the learner to investigate the reasons of the poor fit (by e.g. querying points near the bad fit region), and then improve the model so that the fit is better in that region. This corresponds to the shift from Figure 2 Left to Figure 2 Right, where different data leads to a different reachable hypothesis space. We believe this behaviour is apparent in the SMO experiments we presented for example.

All in all, DEUP does not directly address any shortcoming of discrepancy based measures of EU, except for their assumption that the approximation uncertainty (or bias) is fixed and can thus be ignored. DEUP argues that in practice, (1) such measures are incomplete, and thus, when EU is crucial for decision making (e.g. interactive settings), it might be preferable to use the predicted excess risk as a measure of EU, given that, (2) almost by definition, *it captures both model uncertainty and approximation uncertainty*). We opted for a verbose exposition in Section 2 to actually highlight these two points (1) and (2).


> Ab advantage of DEUP over "discrepancy-based measures of EU" is claimed that it could be adapted to use additional features. I take logical issue with this claim because why would we permit the DEUP model access features withheld from the main model. 
Thank you for raising this point, and we agree that a better wording might be necessary in this sentence. Indeed we could, in principle, use the extra features as inputs to the main model directly, making discrepancy-based measures of EU implicitly rely on them as well. The point we (wrongly) tried to convey by that sentence is what we tried to explain by going from Equation 11 to equation 12: unlike the main predictor (which only cares about x), excess risk is a function of both x and the training dataset, and features conveying information about both can be used as inputs of the excess risk predictor.

> "Perhaps I missed it, but I was disheartened to not see treatment of the model itself as a random variable and how it is a measure of uncertainty.“ Leading to the suggestion suggestion of 
> "more effort dedicated to comparing to / showing the inadequacy of standard assumption validation practices eg Bayesian model criticsm.” 
We agree that we do not provide a theoretical analysis of the adequacy of our proposed estimator of EU under model misspecification. We do agree that it would be a strong contribution, and recent works we referenced ("Minimum excess risk in Bayesian learning.” and "Excess risk analysis for epistemic uncertainty with application to variational inference”) take a stab at that, albeit under strong assumptions. We can highlight this future research direction in the conclusion. 

Thank you for your suggestions to improve the first sentence of the abstract, and sentence about EU decreasing towards 0. We will make sure to include them in the revised version.

Regarding the second sentence of the abstract, we agree that when the model is well specified, it is not merely a proxy, but is an exact measure of EU. Thank you for raising this point. We can simply replace the word “proxy” with “measure”, given that the important part of that sentence is what comes after (the fact that it’s an incomplete measure).

Regarding the “x \mapsto A(x)” comment, we believe that this might just be a notation convention issue. By “x \mapsto A(x)”, we mean “the function A”, as opposed to “A(x)”, which would mean “the value A(x)”. A(x) being equal to \sigma^2(x) is not merely a convention, but is a (simple) consequence of the definitions above.



----------------------------------------------------
>>> Reviewer MM5Y

We would like to thank the reviewer for the thoughtful comments and positive view of the paper! We address your concerns below and will upload a revision with the changes based on your suggestions after the discussion.
 
> It does not refer to original literature on active learning or earlier lit surveys. Gal 2017 is one of the earlier papers that used EU for AL, though QBC (Query-by-Committee) from the 1990s might also count towards that depending on interpretation.

Thanks for mentioning the references! We will add them to the paper in Section 4. 
  
> There are no active learning experiments after setting these expectations: SMO, which seems to me to be the non-Bayesian setting that is also dealt with by Bayesian Optimization, is not active learning per-se.

Thank you for raising this point! We use the term active learning to loosely refer to scenarios where a learning agent can _actively_ make decisions about what data to acquire. This can be in context of traditional active learning where we would like to select datapoints from a pool of unlabelled data to be labelled to improve the learned function, or sequential model optimization where we would like to find the maxima of a black box function. Our focus is mainly on the latter, and we will clarify this in text by referring to it as "interactive learning" to avoid confusion.  

> Algorithm 3's caption reads to be for the "active learning" setting, but it is generally used, while Algorithm 1 does not seem to be used by the paper experiments at all?

As mentioned in the above answer, we will be changing the references to "active learning" with "interactive learning" to avoid confusion. Algorithm 1 is actually used in the OOD Detection experiments in Section 5.3.2 where we would like to learn an uncertainty estimator given a fixed dataset and use it to detect difficult OOD examples, as well as in the illustrative example of Figure 1. We will make this clear in text. Thanks for mentioning this point!

> Figure 2 (right) seems "wrong": H' should stay the same or become smaller with more data. If H is the universe of possible model functions, then it should stay the same. If we look at it from a Bayesian perspective (as a level set in posterior space) then it should become smaller. Imo, the important part is that should move closer to as more data is used for training. (I still need to read Arpit 2017, but it might cause less cognitive dissonance if H' just remained as H.)

It is true that the Bayesian posterior (or more generally the set of hypotheses compatible with the data) should shrink with more data. However, here H and H' represent the set of hypotheses considered before training, i.e., the prior in a Bayesian sense. When more data is available, it is a well-known result from learning theory that the optimal capacity increases, i.e., a larger prior hypothesis space (H' > H) allows better generalization because we have more chances to find a function in H' closer to the ground truth f*. There is of course a trade-off (between bias and variance), but as the amount of data increases, the optimal trade-off implies greater capacity and smaller bias since the increased amount of data pushes variance down.
In addition, with neural networks, there is a notion of effective capacity that factors in the effect of the SGD training procedure and early stopping: 
the effective capacity (the number of randomly labeled training examples that the network can nail) increases with more training iterations, and a larger dataset generally means that early stopping will occur later, after more iterations, and thus with a larger effective capacity. Hence, SGD-trained neural networks with early stopping perform a form of automatic model selection, with effective capacity (the "size" of the prior) increasing with the amount of data. Nonetheless, to avoid confusion, we have removed the right part of figure 2.


> The definition of epistemic uncertainty as approximation uncertainty + model uncertainty/bias seems to contradict the definition of epistemic uncertainty as reducible uncertainty: commonly, it is reducible by gaining access to more data, not by also changing the model. Hence, the model bias is assumed as fixed usually, is it not? Malinin et al have also decomposed (total) uncertainty into aleatoric, epistemic und model uncertainty in one of their early papers (you are probably better aware of it than I). As such, you might want to consider that you do not actually predict epistemic uncertainty but are looking at proxies for the generalization error.

We agree that traditional analyses of epistemic uncertainty assume the family of functions and thus the model bias to be fixed. However, in models typically used in practice like neural networks, the model bias is not fixed and is in fact reducible (as we tried to argue in Figure 2 and Section 2 and in our above comment) as it is induced by factors such as the optimization procedure (e.g., SGD) and techniques like early stopping. We believe that a key contribution of our work is that it takes into account that the family of function can grow in size (and thus bias be reduced) as more data becomes available, in order to estimate a reducible uncertainty that includes the effect of such bias reductions. 


> In §3.1, the paper enumerates different examples for how to estimate aleatoric uncertainty. It would seem that in the cases that aleatoric uncertainty is set to 0, DEUP would not actually compute EU but total uncertainty or rather predict the full error. This is not epistemic uncertainty.

It is right that DEUP would predict the full error in such settings. But given the decomposition of error in Section 2, we argue that this predicted error can be decomposed into a term corresponding to aleatoric uncertainty plus a term corresponding to epistemic uncertainty, seen as the reducible error with more data and better models (which would lead to a zero error if there was no aleatoric uncertainty). Hence, when aleatoric uncertainty is 0, the total generalization error is solely due to reducible forms of error (i.e., epistemic uncertainty). Again, this is because we include the fact that bias can be reduced as more data is acquired.


> For me, the step from theory (11) to implemented method (12) is not clear and a huge step: in particular, how important is $x$ in the feature vector that is used to train the error predictor? It would seem that it should not be too important because: given that we train the predictor on the future dataset, training samples close to $x$ should be exactly where the model will have better performance next. Yet, usually we add the most informative samples to dataset (with highest EU), so the error will be large for those samples, which means the error predictor will be trained to expect high losses, even though after training the model should have small loss for the newly acquired data. Are the losses updated using the newly trained models? How does this square?

We believe the step from (11) to (12) is actually pretty common (especially in pre-deep learning machine learning), whenever the inputs cannot be used as they are to train a predictor. $\phi_z(x)$ represents hand-designed features of the actual input pair $(x, z)$, where $z$ is a dataset. As usual, whenever we embed the inputs in a feature space, we *lose* information: the embedding with the least amount of information lost is the identity embedding (i.e. using $(x, z)$ as inputs). But there is a trade-off between the informativeness of the chosen features and their usability. Given that $x$ is usually a low-dimensional object (compared to $z$, which is a dataset of $(x, y)$ pairs), it seems natural to use $x$ as is in the feature vector.
To "square" the difference between the error of a novel point (selected by active learning) and a point used as part of the training set, our features $\phi_z(x)$ also include a binary indicator: is x part of the training set z or not? This helps to predict the level of error expected at x.
As confirmed by our SMO experiment, after enough training iterations, the error predictor is able to exploit these features:
If x is close to inputs in the dataset z, then (x, z) corresponds to a low error, i.e. the main predictor trained on z should have a low error at x.
If x is far from the inputs in z, then (x, z) corresponds to a high error.
This is the desired behaviour, and we believe it would be harder to learn it without having $x$ in the features $\phi$, unless there is a risk of overfitting to the $x$ part of $\phi$ and not using the information encoded in the other features. In the OOD detection experiments, we actually do not use $x$ in $\phi$ for this reason.

We tried to explain that we are free to chose which features (including $x$) to use in $\phi$. And we would be happy to hear your suggestion as to how to make the point clearer.


> The proposed method seems related to "A statistical framework for efficient out of distribution detection in deep neural networks" and "Density of States Estimation for Out-of-Distribution Detection", in that it uses several different statistics to predict OOD.

Thank you for suggesting the references! They are indeed related and we will add a discussion about them in Section 4. 


> Why do all other SMO methods perform worse than random? Given that the function is sufficiently smooth, a GP should perform better. Was the length scale chosen correctly?

Keep in mind that "random" means random choice of examples to label, so it is not so weak a method, especially in low-dimensional settings. This is the case only for the toy one-dimensional example in Figure 3, and not in the more interesting multi-dimensional one in Figure 4. GP-EI (or GP-UCB) tends to get stuck in local maxima (our function was specifically designed to have multiple such local maxima), and random acquisition is usually a strong baseline in 1D settings. In Figure 3, for GP experiments, the length scale is optimized at every acquisition step by maximizing the log-likelihood of the available data.

> Actual active learning experiments, given that it is mentioned a lot, and AL != SMO (or edit the paper to reduce the reader's expectations to find these).

Thank you for raising this point. As we mentioned above, we will replace the references to active learning with interactive learning to avoid confusion for the reader.

> Update Figure 2 according to the concerns detailed in the previous section.

Please see our response above.
    
> Mention earlier in the paper that you do not require held-out/OOD data for DEUP. The initial sections make it sound like this is a necessity.

Thank you, we will highlight this point more in the introduction.

> On page 10, there are two mentions of Algorithm 3. It looks like accidental text duplication. Please reword these.

Thanks for point this out, we will fix this in the revision. 

> How is the SRCC computed between ID and OOD data? It would seem that all OOD is equal and should have the same "rank". What is the OOD generalization error between CIFAR-10 and SVHN? (OOD is always wrong?) Please clarify this in the text if possible.

By OOD generalization error between CIFAR-10 and SVHN, we refer to the error (which is the NLL loss in this case) of the classifier trained on CIFAR 10 when evaluated on examples from SVHN (OOD examples), where the "true" labels of the OOD examples correspond to the zero vector, unlike the labels of ID examples corresponding to a one-hot vector.

To compute the SRCC, we compute the true errors on OOD and unseen ID examples using the predictions from the main predictor and the ground truth labels, and compute the correlation of these errors with the predicted uncertainties. So all OOD examples actually would have a different rank based on the error made by the main predictor. On a high level, we use this metrics to establish "how well do the uncertainty estimates correlate with the errors made by the predictor". 

> Appendix sections B and C and potentially others don't use \citep but `\cite'. Please fix this too.

Thank you for pointing this out, we will fix the usage in the appendix. 




==> sections/theory-old.tex <==
Consider a supervised learning algorithm (or learner) $\cal L$ mapping a dataset ${\cal D}$
to a predictive function $\hat{f}={\cal L}({\cal D})$. $\cal L$ 
tries to minimize
the expected value of a supervised learning loss $l(\hat{f}(x),y) \in \R$ under unknown probability measure $P(Y|x)$. In this section, we focus on regression tasks with the squared loss $l(\hat{y}, y) = (\hat{y} - y)^2$, with $y \in \sR$. In Appendix~\ref{appendix:theorygeneral}, we provide the corresponding results for a general loss function, with discrete or continuous outputs.

Recall, that for a predictor $\hat{f}$, the \textbf{expected loss} at $x$ is defined as:
\begin{align}\label{eq:totaluncertainty-old}
    {\cal U}(\hat{f},x) = \int  (\hat{f}(x) - y)^2 dP(y|x).
\end{align}
The expected loss is an unknown scalar, as the learner generally does not have access to the true data distribution $P(Y|x)$. The errors made by any predictor $\hat{f}$ at $x$ are due to both the inherent randomness of $P(Y|x)$ (aleatoric uncertainty) and the lack of knowledge of the predictor that can be tackled by acquiring more information around $x$ (epistemic uncertainty). Because of this natural decomposition of the expected loss, we will derive measures of aleatoric and epistemic uncertainty from the expected loss.

Bayes-optimal predictors $f^*$ satisfy the following equation at every $x$:
\begin{align*}
    \forall \Tilde{y} \in \sR \quad \int (f^*(x) - y)^2 dP(y|x) \leq  \int  (\Tilde{y} - y)^2 dP(y|x).
\end{align*}
They depend on the underlying data distribution only and not on learner $\cal L$ or trained predictor $\hat{f}$. Additionally, for any $x$, all  Bayes-optimal predictors have the same total uncertainty at that $x$. The error made by a Bayes-optimal predictor is irreducible and we define it as a measure of the aleatoric uncertainty, which we will denote as:

\begin{align}
  {\cal A}(x) = {\cal U}(f^*,x). 
\end{align}

Because $\mathcal{A}$ is the irreducible part of the expect loss, the remaining part indicates how far a learner is from a Bayes-optimal predictor, or equivalently, how much more there is to learn with more data. It can thus be seen as a measure of epistemic uncertainty of a predictor $\hat{f}$. We will denote it as:

\begin{align} \label{eq:epistemic}
    {\cal E}(\hat{f},x) = {\cal U}(\hat{f},x) - {\cal A}(x) = {\cal U}(\hat{f},x) - {\cal U}(f^*,x).
\end{align}

In the usual regression setting with Gaussian ground truth, the following proposition illustrates why $\mathcal{A}$ and $\mathcal{E}$ are measures of aleatoric and epistemic uncertainty respectively. The proof is provided in Appendix~\ref{appendix:proofs}.
\begin{proposition}
\label{epistemic_mse}
In a regression task with Gaussian ground truth $P(y|x) = \gN(y; \ f^*(x), \ \sigma^2(x))$,
\begin{align*}
    &{\cal E}(\hat{f},x) = (\hat{f}(x) - f^*(x))^2
    \\
    &{\cal U}(\hat{f},x) = \mathbb{E}_{P(y|x)}[(\hat{f}(x) - y)^2] = (\hat{f}(x) - f^*(x))^2 + \sigma^2(x)
    \\
    &{\cal A}(x) = \mathbb{E}_{P(y|x)}[(f^*(x) - y)^2] = \sigma^2(x)
\end{align*}

\end{proposition}

There are several connections here to highlight \emph{why} this measure is useful for active learning settings. Specifically, the expected loss under the distribution of the model matches the A-optimal criterion for model selection \citep{Luter1974ExperimentalDI,zhou2003bayesian}. With the negative log-likelihood loss (Appendix \ref{appendix:theorygeneral}), the corresponding measure of epistemic uncertainty is intimately linked to the Expected Information Gain (EIG), extensively used in the Bayesian Optimal Experimental Design (BOED) literature (See e.g. \citep{pmlr-v89-kleinegesse19a}).

\begin{wrapfigure}{l}{0.5\textwidth}
\vspace*{-4mm}
\begin{center}
\centerline{\resizebox{4.5cm}{!}{\input{figs/bias_variance_bis}}}

\caption{\sl Illustrating noise and bias. Observed $y$ is independent noise plus true $\mathbb{E}[Y|x]=f^*(x)$, itself best approximated by unknown $\tilde{f}(x)$ in parametric set $S$ (orange), e.g., using Bayesian posterior distribution $p(f|\mathcal{D})$ (grey) over parameters. $\tilde{f}$ is the closest function in $S$ to $f^*$, leading to a bias $b(x) = f^*(x) - \tilde{f}(x)$. 
    $\varepsilon(\hat{f})(x)=f^*(x)-\hat{f}(x)$ is the reducible error of the main predictor $\hat{f}$ (e.g. posterior mean),
    whose square corresponds to EU or lack of knowledge, that DEUP aims at estimating.
    With $\tilde{f}$ the unknown ideal predictor and $\hat{f}$ the actual (e.g. mean) predictor, the square of $\Delta f(x) = \tilde{f}(x) - \hat{f}(x)$ induces  
    variance in the posterior. $\varepsilon(\hat{f})(x) = b(x) + \Delta f(x)$ indicates that using the variance as a proxy for EU misses out a non-negligible quantity: the  bias $b(x)$. 
    }
\label{fig:bias-variance-error}
\end{center}
\vspace*{-10mm}
\end{wrapfigure}
\textbf{Relation to existing notions of EU:} Consider a parametric model $p(Y|x, \theta)$ and a learner maintaining a distribution over parameters $\theta \in \Theta$, each corresponding to a predictor $f$ in a parametric set of functions $S$, possibly starting from a prior $p(\theta)$ that would lead to a posterior distribution $p(\theta| \mathcal{D})$. Clearly, the fact that multiple $\theta$'s and corresponding values of $f$ are compatible with the data and the prior indicates lack of knowledge. Because the lack of knowledge indicates where an interactive learner should acquire more information, this justifies the usage of dispersion measures, such as the variance or the entropy of the posterior predictive, as proxies for EU. 

However, the limited capacity of $S$ or the prior $p(\theta)$ may keep the optimal $\tilde{f}$ in $S$ at a distance from the Bayes-optimal predictor $f^*$. We can refer to these self-imposed constraints as a form of bias, in the sense that the learner is usually biased towards the prior preferences,  e.g., towards smoother predictors (typically more so when the dataset is smaller).
This arises when training neural networks with limited data, where the network may not use all of its capacity due to implicit (and not fully understood) regularization properties of SGD~\citep{Kale2021SGDTR}, explicit regularization, early stopping or a combination of these, which can induce a preference on the functions it learns. In Fig.~\ref{fig:bias-variance-error}, we illustrate this gap with the bias function $b(x) = f^*(x) - \tilde{f}(x)$. Because of this bias, model variance cannot be an accurate measure of EU $\mathcal{E}(\hat{f}, x)$ in the general case. % as demonstrated in Fig.~\ref{fig:gpvardeup}.

In Deep Ensembles \citep{lakshminarayanan2016simple}, for example, if all the networks in the ensemble tend to fail in systematic (i.e. potentially reducible) ways, this aspect of prediction failure will not be captured by variance. Whereas Deep Ensembles variance provides us uncertainty regarding which of the networks we could draw is best, this does not tell us how poor that network is even in a noise-free setting. On the other hand, with flexible models like neural networks, adding examples around $x$ where $b(x)^2$ is large may allow to increase capacity around $x$ and reduce $b(x)^2$. 

==> tmlr-rebuttal-todo <==
Changes to make based on reviews:
Reviewer iZLw
> Clarify wording on extra features for error predictor (equation 11 to equation 12)

[Done] > Add future work - theoretical guarantees 

[Done] > Changes in abstract 

Reviewer MM5Y
[Done]> Add references Gal 2017 is one of the earlier papers that used EU for AL, though QBC (Query-by-Committee) from the 1990s 

[Done]> Change references to active learning to interactive learning

[Done] > Clarify Algorithm 1 is used in Fig 1 and OOD experiments. 

[Done] > Add references "A statistical framework for efficient out of distribution detection in deep neural networks" and "Density of States Estimation for Out-of-Distribution Detection", in that it uses several different statistics to predict OOD.

[Done] > Mention earlier in the paper that you do not require held-out/OOD data for DEUP. The initial sections make it sound like this is a necessity.

[DOne] > Page 10 (before section 3) multiple references to Algo 3. Remove one 

[Done] > \citep in Appendix 

Reviewer TayB

> in the paragraph following Eq. 8, in which we argue that an estimator the ER can be used as an estimator of the EU, we explain that this is the case only for agents whose action space allow them to adapt their effective capacity to the dataset (because of SGD e.g.)? 
